Vision-Language Models for Criterion-Level Grading of Handwritten Examinations in Outcome-Based Education

Criterion-level grading connects examination performance to learning outcomes, but manual marking introduces workload and variation between markers. This study evaluates vision-language models (VLMs) for handwritten outcome-based assessment across five dimensions: accuracy, human agreement, repeated-run reliability, error concentration, and explanation quality. Using 1,982 criterion-level records from 485 undergraduate examination answers, we compare 20 configurations spanning Qwen2.5-VL, InternVL3, Pixtral, a Donut baseline, and a cascade ensemble. Evaluation setups include zero-shot prompting, few-shot prompting, partial fine-tuning, and Low-Rank Adaptation (LoRA). Two independent faculty markers regraded all 291 test criteria, providing a human agreement baseline on the same assessment materials. Qwen2.5-VL with LoRA achieved Quadratic Weighted Kappa (QWK) of 0.727 and mean absolute error of 0.435 marks against the examiner, compared with mean human-pair QWK of 0.551. This comparison reflects calibration to the examiner's training marks. LoRA outperformed partial fine-tuning for all three instruction-tuned VLMs, while few-shot prompting reduced QWK in every configuration with valid prompted scores. Aggregate reliability and exact repeatability diverged: intraclass correlations ranged from 0.790 to 0.874, yet 50.2-63.6% of criteria changed marks across five sampled runs. Attention-guided deletion showed no statistically significant advantage over random masking, and four faculty reviewers reached no consensus on explanation usefulness. These findings highlight the need for rubric-specific calibration, repeatable scoring, review of consequential errors, and separate validation of explanations. The released evaluation protocol supports criterion-level assessment research and grading tools with teacher oversight.

==> Tables/tab_fairness.tex <==
\begin{table}[!t]
\centering
\caption{Parse coverage by subject and learning setup for the OCR-free control, the only system in the grid that fails to produce a mark on some records. $n_{\text{tot}}$ is the number of criterion-level judgments offered and $n_{\text{val}}$ the number from which a mark could be recovered.}
\label{tab:fairness}
\vspace{-6pt}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabular}{lrrrrrrr}
\hline
 & & \multicolumn{2}{c}{\textbf{Zero-/few-shot}} & \multicolumn{2}{c}{\textbf{LoRA}} & \multicolumn{2}{c}{\textbf{Full FT}} \\
\textbf{Subject} & $n_{\text{tot}}$ & $n_{\text{val}}$ & \% & $n_{\text{val}}$ & \% & $n_{\text{val}}$ & \% \\ \hline
Machine Learning & 36 & 0 & 0 & 20 & 56 & 22 & 61 \\
Digital Image Processing & 28 & 0 & 0 & 20 & 71 & 21 & 75 \\
Database Systems & 64 & 0 & 0 & 36 & 56 & 23 & 36 \\
Computer Networks & 45 & 0 & 0 & 17 & 38 & 39 & 87 \\
Data Mining & 32 & 0 & 0 & 22 & 69 & 14 & 44 \\
Algorithms & 40 & 0 & 0 & 14 & 35 & 12 & 30 \\
Fisheries & 18 & 0 & 0 & 12 & 67 & 1 & 6 \\
Object Oriented Prog. & 20 & 0 & 0 & 9 & 45 & 14 & 70 \\
\hline
\textbf{Total} & \textbf{283} & \textbf{0} & \textbf{0} & \textbf{150} & \textbf{53} & \textbf{146} & \textbf{52} \\
\hline
\end{tabular}
\end{table}

